Precise, Dynamic Information Flow for Database-Backed Applications

We present an approach for dynamic information flow control across the application and database. Our approach reduces the amount of policy code required, yields formal guarantees across the application and database, works with existing relational database implementations, and scales for realistic applications. In this paper, we present a programming model that factors out information flow policies from application code and database queries, a dynamic semantics for the underlying {\lambda}^JDB core language, and proofs of termination-insensitive non-interference and policy compliance for the semantics. We implement these ideas in Jacqueline, a Python web framework, and demonstrate feasibility through three application case studies: a course manager, a health record system, and a conference management system used to run an academic workshop. We show that in comparison to traditional applications with hand-coded policy checks, Jacqueline applications have 1) a smaller trusted computing base, 2) fewer lines of policy code, and 2) reasonable, often negligible, additional overheads.

==> discussion.tex <==
\section{Discussion}
In this section we discuss issues related to security and choice of language and web framework.

%That said, using a web framework like \webframework{} can prevent many of the issues that security papers often discuss.
%For instance, using Django and other web frameworks properly can prevent common security vulnerabilities such as unauthorized password disclosure, directory traversal, file access control issues, and various SQL injection and cross-site scripting attacks. Because \webframework{} builds even more controls on top of this, \webframework{} prevents even more vulnerabilities. Specifically, \webframework{} takes responsibility for propagating policies, eliminating possible errors from missing access checks.

%The \webframework{} web framework also mitigates some potential sources of programmer error with Jeeves. In Jeeves, the programmer is responsible for providing the output channel corresponding to the principal viewing the data. \webframework{} helps manage the viewer, making it less likely there is an error with specifying this information. \TODO{Come up with more situations.}

\subsection{Decision to Use Python}
We had considered implementing \webframework{} in Scala, a language for which there already exists an implementation of Jeeves~\cite{FacetPaper}, but we chose Python because the dynamic approach of Jeeves fits more with the Python's dynamic programming idioms. Jeeves's policy-agnostic approach trades developer overhead for runtime overhead, making it more suitable for rapid prototyping and for building web applications at a smaller scale. While Scala is gaining increasing traction in industry and is in use at companies like Twitter and LinkedIn, it has not been the language of choice for the casual programmer building a recreational web application.

The biggest difference in the approach to embedding a language in Python is that while Scala is statically typed, Python is dynamically typed. Scala's static types make the programmer think more carefully and be more verbose in the implementation. The trade-off is that the static types provide more guarantees about the cases that the implementation covers, making it more crucial to thoroughly test the code. Both Python and Scala allow for most, but not all, operators to be overloaded. With Scala, a work-around is to use compiler extensions like Scala-Virtualized~\cite{ScalaVirtualized} that allow programmers to overload key constructs. With Python, we were able to work around the lack of full overloading by doing a source transformation. In Python, this was straightforward because the AST is relatively simple and the Python MacroPy library~\cite{Macropy} for implementing macros provides support.

%One issue we ran into with the Scala embedding was that the programmer is required to fully annotate the faceted types. One of the goals of creating a policy-agnostic approach is to allow the programmers to write programs similar to the ones they would have written before while handling privacy under the covers. An issue with the Scala implementation is that the programmer needs to annotate all of the programs with the faceted versions of the types. \TODO{Also, because there are some gaps with the implementation, the programmer is painfully aware of the fact that they are not writing in vanilla Scala...}

%Both the Scala and Python implementations preserve the Jeeves guarantees. Since Jeeves takes a fully dynamic approach, the non-interference guarantees about high values flowing only to viewers with restricted access hold in both implementations. The guarantees that the Scala and Python implementations enforce are the same, but the Scala DSL enforces typing rules at compile time, while the Python DSL enforces the rules at run time.

%\subsection{Decision to Use Django}
%Our web framework is currently an ad hoc layer on top of Django. We decided to use Django because it is a well-known web framework with support for a variety of functionality. It turned out that we needed to customize nearly all of Django's functionality that we used. Thus, a more lightweight framework may be a more optimal choice for the base web framework.

%Ideally, we would also modify the templating engine to support facets. Conceptually, a view would return some sort of faceted response object. In addition, the templating system should handle keeping track of the viewer and concretizing things so the programmer does not have to do so explicitly.

\subsection{Comparison of the Conference Management System to HotCRP}
We compare our implementation to the implementation of HotCRP, a state-of-the-art conference management system. HotCRP is an excellent example of the ``policy spaghetti'' that \webframework{}'s design is intended to mitigate. Policy code pervades the entire HotCRP codebase. Because the programmer needs to manage policies and access checks, almost all of the PHP files need to be policy-aware.

The anatomy of the HotCRP policy code is as follows. The HotCRP policies are implemented in across at least 24 of the 82 PHP files. Many policy functions are contained in file \code{contact.php} and other files call these functions when determining what may be shown.
There are additional checks across the program. For instance, there are 191 occurrences of checks involving the \code{privChair} and \code{conflictType} variables checking whether the viewer is the PC chair or has the appropriate conflict status.
There is also a fair amount of policy code associated with SQL queries: many SQL queries construct \sql{WHERE} clauses with conditions based on policies.
The policy code is at least $2,322$ out of $42,006$ total lines of code. There are over $500$ calls to policy functions across $24$ files.

We show an estimated lower bound on the lines of ``policy code'' in Table~\ref{tab:hotcrp_loc}. We define policy code as code involved in access checks or defining functions used in these checks. The numbers are an underestimate: we counted the functions defined in \code{contact.php}, their uses, and the appearance of a few other variables known to be used for access checks. There are dynamically-generated SQL queries across the code. The policy code is at least $2,322$ out of $42,006$ total lines of code. There are over $500$ calls to policy functions across $24$ files.

Though HotCRP has more features and more complex policies than our \webframework{} conference management system, the main take-away is that there is policy code scattered across the code base.
It is difficult to even characterize what counts as ``policy code'' because it is so intertwined with functionality.
Designing a privacy API on top of the database could mitigate some of these issues, and having a domain-specific privacy language could reduce the number of lines of policy code.
ven with more careful system design and abstraction, privacy would remain a global concern and the programmer remains responsible for making checks across the code base.
In such a system, the trusted base for the policy code must be the entire code base.

\begin{table}
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Language} & \textbf{Files} & \textbf{Code} & \textbf{Estimated Policy}\\
\hline
\hline
PHP & 82 & 34889 & $>$2326 \\
JavaScript & 4 & 2566 & 0\\
CSS & 1 & 2503 & 0\\
Perl & 4 & 1422 & 0\\
SQL &  1 & 389 & many\\
C++ & 1 & 237 & 0\\
\hline
Total & -- & 42006 & $\gg$2322 (5.5\%)\\
\hline
\end{tabular}
\caption{Lines of code and estimated lines of policy in HotCRP.}
\label{tab:hotcrp_loc}
\end{table}



==> faceted_evaluation_semantics.tex <==
\begin{figure*}\caption{Faceted evaluation semantics.{}\label{fig:fvSem}\label{fig:runSyn}\label{fig:refUtils}}
\footnotesize
{\bf Runtime Syntax}
%\footnotesize
\[
\begin{array}{rclcl}
        e	                \quad &\in\quad & \fun{Expr}	\quad &::=  & \quad ... ~|~ a \\
	\Sigma	        \quad &\in\quad & \fun{Store}	\quad &=  & \quad (\fun{TableName} \rightarrow_p Value)
                  ~\cup~ (\fun{TableName} \rightarrow (FieldName \rightarrow (\fun{Value} \times \fun{Value})))
                  ~\cup~ (\fun{Label} \rightarrow \fun{Value}) \\
                  %\cup \fun{Value}  \\

	%\Theta	        \quad &\in\quad & \fun{Subst}	\quad &=  & \quad \fun{Var} \rightarrow_p \fun{Value} \\
	R		\quad &\in\quad & \URawValue	\quad &::=& \quad c ~|~ t ~|~ \lamc{x}{\ue} \\
	%LT		\quad &\in\quad & \fun{LabelType}	\quad &::=& \quad \confLabel ~|~ \intLabel \\
	a		\quad &\in\quad & \fun{Address} \\
	%c		\quad &\in\quad & \fun{Constants}	\quad &::=& \quad f ~|~ ... \\
	%D		\quad &\in\quad & \DataItem	\quad &::=& \quad \dataOut{\pc}{V}{v} \\
	\uv		\quad &\in\quad & \UValue	\quad &::=& \quad R ~|~ \labval{k}{V_1}{V_2} \\ 
	h		\quad &\in\quad & \USignedLabel	& ::= & \quad k ~|~ \notlab k \\
	\pc		\quad &\in\quad & \mathit{PC} &=& \quad 2^\USignedLabel \\~\\
\end{array}
\]
{\bf Expression Evaluation Rules~~~ \fbox{$\sstep \Sigma e {\pc} {\Sigma'} V$}}
\\
\[
%\begin{array}[t]{@{\!\!\!\!\!\!\!\!\!\!}cl}
\begin{array}[t]{cl}
\setuprulecol
\mmrule{f-create}{
		\sstep \Sigma e \pc {\Sigma_r} V_r \\
    V_r = \{ f = V_f \}\\
    \Sigma_r(n)(f) = (e_p, e_d)\\
    k \not\in \fun{dom}(\Sigma')\\
    \sstep {\Sigma_r} {\policy{k}{e_{p}~V_r}} \pc {\Sigma_p} V_{p}\\
    \sstep {\Sigma_p} {e_{d}~V_r} \pc {\Sigma'} {V_{d}}\\
    V' = \{ f = \labexpr{k}{V_r}{V_{d}} \}\\
	  \Sigma'' = \dbOp(\Sigma', pc, n, V', dbinsert)
  }{
		\sstep \Sigma {(\create{n}{e})} \pc {\Sigma''} {V'}
	}
\mmrule{f-save}{
          \sstep \Sigma {e} \pc {\Sigma'} V_r\\
          V_r = \{ f = V_f \}\\
    \Sigma_r(n)(f) = (e_p, e_d)\\
    k \not\in \fun{dom}(\Sigma')\\
    \sstep {\Sigma_r} {\policy{k}{e_{p}~V_r}} \pc {\Sigma_p} V_{p}\\
    \sstep {\Sigma_p} {e_{d}~V_r} \pc {\Sigma'} {V_{d}}\\
    V' = \{ f = \labexpr{k}{V_r}{V_{d}} \}\\
                \Sigma'' = {\dbOp}(\Sigma', \pc, n, V', dbupdate)
	}{
		\sstep \Sigma {\save{n}{e}} \pc {\Sigma''} {V'}
	}
\mmrule{f-select}{
          \sstep \Sigma e \pc {\Sigma'} V \\
         V' = {\selectOp}(\Sigma',p,V,\pc)
  }{
    \sstep \Sigma {\select{p}{e}} \pc {\Sigma'} V'
  }
\end{array}
\qquad\qquad
\begin{array}[t]{cl}
\setuprulecol
\mmrule{f-val}{
  }{
    \sstep \Sigma R {\pc} \Sigma {R} 
  }
\mmrule{f-app}{
        	\sstep \Sigma {e_1} \pc {\Sigma_1} V_1 \\
        	\sstep {\Sigma_1} {e_2} \pc {\Sigma_2} V_2 \\
               \appstep {\Sigma_2} {V_1 ~V_2} \pc {\Sigma'} {V'}
      }{
        	\sstep \Sigma {(e_1~e_2)} \pc {\Sigma'} {V'}
        } 
\mmrule{f-split}{
		k \not\in\pc~ \mbox{ and } \notlab k \not\in\pc \\
		\sstep {\Sigma} {e_1} {\joinLab k \pc} {\Sigma_1} {V_1} \\
		\sstep {\Sigma_1} {e_2} {\joinLab {\notlab k} \pc} {\Sigma'}{V_2} \\
    V' = {\labResult{k}{V_1}{V_2}} \\
	}{
		%\sstep \Sigma {\labexpr{k}{e_1}{e_2}} \pc {\Sigma'} {\labResult{k}{V_1}{V_2}}
		\sstep \Sigma {\labexpr{k}{e_1}{e_2}} \pc {\Sigma'} {V'}
	}
\mmrule{f-left}{
		k \in\pc \qquad
		\sstep \Sigma {e_1} \pc {\Sigma'} {V} \\
	}{
		\sstep \Sigma {\labexpr{k}{e_1}{e_2}} \pc {\Sigma'} V
	}
\mmrule{f-right}{
		\notlab k \in\pc \qquad
		\sstep \Sigma {e_2} \pc {\Sigma'} {V} \\
	}{
		\sstep \Sigma {\labexpr{k}{e_1}{e_2}} \pc {\Sigma'} V
	}
\end{array}
\]
\vskip -.2in
\[
\begin{array}[t]{cl}
\setuprulecol
\mmrule{f-record}{
    \sstep \Sigma e \pc {\Sigma'} V
  }{
    \sstep \Sigma {\{ f = e \}} \pc {\Sigma'} {\{ f = V\}}
  }
\mmrule{f-label}{
                k' fresh \\
        	\sstep {\Sigma[k':=\lam x \true]} {e[k:=k']} \pc {\Sigma'} V \\
	}{
		\sstep \Sigma {\levelDecl k e} \pc {\Sigma'} V'
	}
\mmrule{f-restrict}{
    \sstep \Sigma e \pc {\Sigma_1} V \\
    \Sigma' = \Sigma_1[k:=\Sigma_1(k)\policyAdd \labResult{\joinLab{k}{\pc}}{V}{\lam x \true}] \\
    %\Sigma' = \Sigma_1[\policyVar := (\policyStore{\Sigma_1} \policyAdd {\labResult {\joinLab{pc}{k}} V {\lam x \true}})]
  }{
		\sstep \Sigma {\policy k e} {\pc} {\Sigma'} {V}
  }
\mmrule{f-table}{}{
    \sstep \Sigma {\tableDecl{n}{\{f: (e_{p}, e_{d})\}}} {\pc} {\Sigma(n)[f := (e_p, e_d)]} {t}
}
\end{array}
\]
{\bf Auxiliary Functions}
%\footnotesize
\[
\begin{array}{lcl}
\selectOp\funtype{\fun{Store}\times\UValue\times\UValue\times\mathit{PC}}{\UValue} \\
{\selectOp}(\Sigma,p,t,\pc) & = & dbselect(p, t) \\
{\selectOp}(\Sigma,p,\labval k {\Vhigh } {\Vlow }, \pc) & = & \left\{
\begin{array}{ll}
{\selectOp}(\Sigma,p,\Vhigh,\pc)  & \mbox{if } k \in \pc \\
{\selectOp}(\Sigma,p,\Vlow,\pc)  & \mbox{if } \notlab k \in \pc \\
\labexpr{k}{{\selectOp}(\Sigma,p,\Vhigh,\pc)} {{\selectOp}(\Sigma,p,\Vlow,\pc)}  & \mbox{otherwise} \\
\end{array} \right. \\
\end{array}
\]
\\
%%
\[
\begin{array}{lcl}
\facetOp\funtype{\UValue \times\mathit{PC}\times Name \times \UValue \times ((\UValue \times \UValue) \rightarrow \UValue)}{\UValue} \\
\facetOp(V_t,pc,n,V,op) & = & \labResult{pc}{op(V_t, V)}{V_t}\\
\facetOp(\labval{k}{V_H}{V_L},pc,n,V,op) & = & 
 \left\{
\begin{array}{ll}
{\facetOp}(V_H,\pc,n,V,op)  & \mbox{if } k \in \pc \\
{\facetOp}(V_L,\pc,n,V,op)  & \mbox{if } \notlab k \in \pc \\
\labval{k}{\facetOp(V_H, pc, n, V, op)}{\facetOp(V_L, pc, n, V, op)}
& \mbox{otherwise} \\
\end{array} \right. \\
\end{array}
\]
\\
%%
\[
\begin{array}{lcl}
\dbOp\funtype{\fun{Store}\times\mathit{PC}\times Name \times \UValue \times ((\UValue \times \UValue) \rightarrow \UValue))}{\fun{Store}} \\
{\dbOp}(\Sigma,pc,n,V,op) & = & \Sigma[n := \facetOp(\Sigma (n), pc, n, V,op)]\\
{\dbOp}(\Sigma,pc,n,\{ f = \labval k {\Vhigh}{\Vlow} \}, op) & = & \Sigma' 
\qquad\begin{array}[t]{l}
  \mbox{ where } \Sigma_1 = {\dbOp}(\Sigma,~\,\joinLab k \pc,n, \{ f = \Vhigh \}) \\
    \mbox{ and }  \,~~~\Sigma'~ = {\dbOp}(\Sigma_1,\joinLab {\notlab k} \pc, n, \{ f = \Vlow \}) \\
    \end{array}\\
\end{array}
\]
\end{figure*}
%\vskip .1in


==> jacqueline_web.tex <==
\subsection{The \webframework{} Web Framework}
\begin{figure}
\begin{lstlisting}[language=Python, xleftmargin=10pt, numbers=left, escapeinside={~}{~}]
class Event(Model):
  VISIBILITY = (('E', 'Everyone')
    , ('G', 'Guests' ))

~\label{lst:calendar_name}~  name = CharField(max_length=256)
  location = CharField(max_length=512)
  time = DateTimeField()
  description = CharField(max_length=1024)
  visibility = CharField(max_length=1
    , choices=VISIBILITY, default='E')

  # Public value for name field.
  @staticmethod
~\label{lst:calendar_public}~  def jeeves_get_public_name(event):
    return "Private event"

  # Policy function for name field.
  @staticmethod
  @label_for('name')
  @jeeves
~\label{lst:calendar_policy}~  def jeeves_restrict_event(event, ctxt):
    if event.visibility == 'G':
      return EventGuest.objects.get(
        event=self, guest=ctxt) != None
    else:
      return True

~\label{lst:calendar_EventGuest}~class EventGuest(Model):
  event = ForeignKey(Event, null=True)
  guest = ForeignKey(UserProfile, null=True)
\end{lstlisting}
\caption{\webframework{} schema fragment for calendar events.}
\label{fig:calendar_code}
\end{figure}

Information flow policies determine whether the sensitive or public value flows to an output context. On line~\ref{lst:calendar_policy} we implement the information flow policy determining when the sensitive \python{name} field may flow to viewers. The policy queries the database, looking up in the \python{EventGuest} table (line~\ref{lst:calendar_EventGuest}) whether a given guest is associated with the event. Policies take two arguments, the current row and the viewer, and return a Boolean expression that may depend on sensitive values.

\webframework{} allows the programmer to write \emph{policy-agnostic} code. 
For instance, the code to get all guests can simply be the following:
\begin{lstlisting}
guest_events = EventGuest.objects.filter(
  guest=profile).all()
\end{lstlisting}
The programmer does not need to check the permissions of the event (whether it's ``everyone'' or ``guests only'') or to which viewer \python{guest_events} or a derived value is being shown. \webframework{} keeps track of the output context, associated with a session, in order to show the result appropriately.

\subsection{Object-Relational Mapping}
We extend Django's ORM to allow the programmer to specify policies on the models and to augments tables with additional columns to track labels. We implemented \python{JeevesModel}, a subclass of Django's \python{Model}, to support a subset of the API of Django's ORM, including \python{get} and \python{filter}. Our implementation handles joins and foreign keys. The ORM has a standardized naming scheme for labels in order to uniquely identify associated objects and policies.



==> jelf_ast.tex <==
\newcommand{\jelfRow}{r}
\newcommand{\jelfTable}{\mathcal{T}}
\newcommand{\jelfExp}{e}
\newcommand{\jelfStmt}{Stmt}
\newcommand{\jelfSchema}{Schema}
\newcommand{\queryPredicate}{q}
\newcommand{\jelfPolicy}{p}
\begin{figure*}
\centering
%$\begin{array}{l@{\quad}c@{\quad}l@{\qquad\quad}r}
$\begin{array}{l@{\qquad}c@{\qquad}l@{\qquad\qquad\quad}r}
%%% Honest-to-goodness values
%%% Operations on the constraint environment
x, p, \tau, \ell & & & \t{variables, primitives, types, labels}\\
s, f & & & \t{schema names, data fields} \\
\mathcal{L} & ::= & \b{low} \ors \b{high} & \t{labels}\\
\queryPredicate & ::= & f \ (op) \ \jelfExp \ors \jelfExp \ (op) \ f & \t{query predicates}\\
\jelfRow & ::= & \{ \overline{f = \jelfExp} \} & \t{database rows}\\
\jelfTable & ::= & s \ors \jelfRow \ \b{list} \ors \b{select} \ \overline{f} \ \b{from} \ \jelfTable \ (\b{where} \ \overline{\queryPredicate}) & \t{database tables} \\
& \ors & \b{join} \ \jelfTable_1 \ \jelfTable_2 \ors \jelfTable \ \b{orderby} \ \overline{f}\\
%  & \ors & \b{filter} (\jelfTable, \overline{\queryPredicate}) \ors \b{get} (\jelfTable, \overline{\queryPredicate})\\
\jelfExp & ::= & x \ors p \ors r & \t{expressions}\\
    & \ors & \lambda x: \tau . \jelfExp \ors \jelfExp_1 \ \jelfExp_2 \ors \jelfExp_1 \ (\t{op})\ \jelfExp_2 \ors \jelfExp_1 ; \ \jelfExp_2\\
    & \ors & \b{if} \ \jelfExp_c \ \b{then} \ \jelfExp_t \ \b{else} \ \jelfExp_f \ors \b{let} \ x = \jelfExp_1 \ \b{in} \ \jelfExp_2\\
%    & \ors & \langle \ell \ ? \ \jelfExp_{high} \ : \ \jelfExp_{low} \rangle & \t{faceted values}\\
    & \ors & \jelfRow \ors \b{create}(s, \jelfRow) \ors \b{save}(s, \jelfRow) \ors \jelfExp.f \ors \b{for} \ x \ \b{in} \ \jelfTable \ \b{do} \ \jelfExp & \t{integrated queries}\\
% statements
\jelfStmt & ::= & \b{let} \ x = \jelfExp \ \b{in} \ \jelfStmt& \t{statements}\\
    & \ors & \b{print} \ \{ \jelfExp_c \} \ \jelfExp\\
p & ::= & \{ \b{flowsto} \ \lambda (x_r, x_c).\jelfExp_p; \ \b{public} \ \lambda x_r.\jelfExp_d \} & \t{policies}\\
\jelfSchema & ::= & \b{schema} \ s : \ \overline{f: \tau \ (p)} \ (\b{where} \ (x = e)^*)^+ & \t{schemas}\\
Program & ::= & \jelfSchema^* \ \jelfStmt^+ & \t{program}\\
\end{array}$
\caption{\dblang{} syntax.}
\label{fig:jelfsyntax}
\end{figure*}


==> jinq_evaluation_contexts.tex <==
\newcommand{\ctxthole}{~\bullet~}

\begin{figure}
\centering
{\bf Evaluation Contexts}
\[
\begin{array}{l@{\qquad}c@{\qquad}l@{\qquad\qquad\quad}}
E &::=& \labval{k}{E}{e} \ors \labval{k}{V}{E}\\
  &\ors& \ctxthole \ e \ors v \ \ctxthole \ors \mkref \ctxthole \ors \deref \ctxthole \ors \assign \ctxthole e \ors \assign V \ctxthole\\
  &\ors& \row {V \dots \ctxthole e \dots} \ors \select{i}{j}{\ctxthole} \ors \project{\overline{i}}{\ctxthole}\\
  &\ors& \join{\ctxthole}{e} \ors \join{v}{\ctxthole} \ors \union{\ctxthole}{e} \ors \union{V}{\ctxthole}\\
  &\ors& \fold{\ctxthole}{e}{e} \ors \fold{V}{\ctxthole}{e} \ors \fold{v}{v}{\ctxthole}\\
\end{array}
\]
{\bf Strict Contexts}
\[
\begin{array}{l@{\qquad}c@{\qquad}l@{\qquad\qquad\quad}}
S &::=& \ctxthole \ e \ors \deref \ctxthole \ors \assign{\ctxthole}{V} \ors \select{i}{j}{\ctxthole} \ors \project{i}{\ctxthole}\\
  &\ors& \join{\ctxthole}{V} \ors \join{\jtable T}{\ctxthole} \ors \union{\ctxthole}{V} \ors \union{\jtable{T}}{\ctxthole}\\
  &\ors& \row {S \dots \ctxthole \dots e} \ors \fold{V}{V}{\ctxthole}\\
\end{array}
\]
\caption{Evaluation with contexts.}
\label{fig:evaluation_ctxts}
\end{figure}


==> jinq_semantics_old.tex <==
\begin{figure*}\caption{Faceted evaluation of \dblang without relational operators.\label{fig:fvSem}\label{fig:runSyn}\label{fig:refUtils}}
%\footnotesize
\input{standard_facet_rules_old}
\end{figure*}

\begin{figure*}\caption{Faceted evaluation with relational operators.}\label{fig:relOps}
\[
\begin{array}[t]{cl}
\setuprulecol
% F-ROW
\mmrule{f-row}{
  }{
    \sstep \Sigma {\row{\overline{s}}} {pc} \Sigma {(\jtable{(\epsilon, \overline{s})})}
  }
% F-SELECT
\mmrule{f-select}{
    T' = \{ (B, s_1 \dots s_n) \in T ~|~ s_i = s_j \}
  }{
    \sstep \Sigma {\select{i}{j}{(\jtable{T})}} {pc} \Sigma {(\jtable{T'})}
  }
\end{array}
\begin{array}[t]{cl}
\setuprulecol
% F-UNION
\mmrule{f-union}{
  }{
    \sstep \Sigma {\union{(\jtable{T_1})}{(\jtable{T_2})}} {pc} \Sigma {(\jtable{T_1.T_2})}
  }
% F-PROJECT
\mmrule{f-project}{
    \overline{i} = i_1 \dots i_n \qquad
    T' = \{ (B, s_{i_1} \dots s_{i_n}) ~|~ (B, s_1 \dots s_m) \in T\}\\
  }{
    \sstep \Sigma {\project{\overline{i}}{(\jtable{T})}} {pc} \Sigma {(\jtable{T'})}
  }
\end{array}
 \]
\vspace{-.3cm}
\[
\begin{array}[t]{cl}
% F-JOIN
\mmrule{f-join}{
     T_3 = \{ (\union{B_1}{B_2}, s_1 \dots s_m s_1' \dots s_n') ~|~ (B_1, s_1 \dots s_m) \in T_1, (B_2, s_1' \dots s_n') \in T_2 \}
  }{
    \sstep \Sigma {\join{(\jtable{T_1})}{(\jtable{T_2})}} {pc} \Sigma {(\jtable{T_3})}
  }
% F-FOLD-EMPTY
\mmrule{f-fold-empty}{

  }{
    \sstep {\Sigma} {\fold{V_f}{V_p}{(\jtable{\epsilon})}} {pc} {\Sigma} {V_p}
  }
% F-FOLD-INCONSISTENT
\mmrule{f-fold-inconsistent}{
  \sstep {\Sigma} {\fold{V_f}{V_p}{(\jtable{T})}} {pc} {\Sigma'} {V'} \qquad
  B \t{ inconsistent with } pc\\
}{
  \sstep {\Sigma} {\fold{V_f}{V_p}{(\jtable{(B, \jrow{s}).T})}} {pc} {\Sigma'} {V'}
}
% F-FOLD-CONSISTENT
\mmrule{f-fold-consistent}{
  \sstep {\Sigma} {\fold{V_f}{V_p}{(\jtable{T})}} {pc} {\Sigma'} {V'} \qquad
  B \t{ consistent with } pc \qquad
  \sstep {\Sigma'} {V_f~\jrow{s}~V'} {pc \cup B} {\Sigma''} {V''}
}{
  \sstep {\Sigma} {\fold{V_f}{V_p}{(\jtable{(B, \jrow{s}).T})}} {pc} {\Sigma''} {\labResult{B}{V''}{V'}}
}
%%
\end{array}
\]
\end{figure*}


==> lang_source.tex <==
\newcommand{\ue}{e}
\newcommand{\mkref}[1]{\t{ref}~#1}
\newcommand{\deref}[1]{\t{!}#1}
\newcommand{\assign}[2]{#1\t{:=}\,#2}

%\newcommand{\labexpr}[3]{\langle #2 ~|~ #3 \rangle \b{(} #1 \b{)}}
\newcommand{\readFile}[1]{\t{read}(#1)}
\newcommand{\writeFile}[2]{\t{write}(#1,#2)}
\newcommand{\print}[2]{\t{print}~\{#1\}~#2}
\newcommand{\levelDecl}[2]{\t{label}~{#1}~\t{in}~{#2}}

\newcommand{\fh}{f}

\newcommand{\defaultVal}{0}

% encodings
\newcommand{\ife}[3]{\t{if}~{#1}~\t{then}~{#2}~\t{else}~{#3}}
\newcommand{\letin}[3]{\t{let}~{#1}~\t{=}~{#2}~\t{in}~{#3}}

% bool vals
\newcommand{\true}{\fun{true}}
\newcommand{\false}{\fun{false}}

% Specifying policy as a lambda function that returns a boolean value.
\newcommand{\policy}[2]{\t{restrict}(#1,#2)}
\newcommand{\policyStd}[1]{\t{restrict}(#1)}
\newcommand{\policyVar}{policy}
\newcommand{\policyStore}[1]{#1^{policy}}
\newcommand{\policyAdd}{\wedge_f}

\newcommand{\fileOut}[2]{{#1}\!:\!{#2}}

\begin{figure}\caption{The source language \corelang{}.\label{fig:syntax}}
\mbox{}\\
~{\bf Syntax:}
\[
\begin{array}{llr}
        \mydefhead{e ::=\qquad\qquad\qquad\qquad}{Term}
        \mydefcase{x}{variable}
        \mydefcase{c}{constant}
        %\mydefcase{f}{file handle}
        %\mydefcase{\defaultVal}{default value}
        \mydefcase{\lam x e}{abstraction}
        \mydefcase{\ue_1~\ue_2}{application}
        \mydefcase{\mkref e}{reference allocation}
        \mydefcase{\deref e}{dereference}
        \mydefcase{\assign e e}{assignment}
        %\mydefcase{\readFile{e_1}}{file read}
        %\mydefcase{\writeFile{e_1}{e}}{file write}
        %\mydefcase{\labexpr{k}{e_1}{e_2}{\policy{e_p}}}{faceted expression}
        \mydefcase{\labexpr{k}{e_1}{e_2}}{faceted expression}
        \mydefcase{\levelDecl{k}{e}}{label declaration}
        \mydefcase{\policy{k}{e}}{policy specification}
       \\
        \mydefhead{S ::=\qquad\qquad\qquad\qquad}{Statement}
        \mydefcase{\letin{x}{e}{S}}{let statement}
        \mydefcase{\print{e}{e}}{print statement}
        \\
        \mydefhead{c::=}{Constant}
        % \mydefcase{\fh}{file handle}
        \mydefcase{b}{boolean}
        \mydefcase{i}{integer}
\\
        \mydefhead{x,y,z}{Variable}
        \mydefhead{k,l}{Label}
\end{array}
\]
%\\
%~{\bf Standard encodings:}  \label{fig:condPairSyn}
%\[
%\begin{array}{@{}r@{~~~}c@{~~~}l}
        %\true   &\defeq& \lam x {\lam y x} \\
        %\false  &\defeq& \lam x {\lam y y} \\
        %\ife{e_1}{e_2}{e_3} &\defeq&
              %(e_1~(\lam d {e_2})~(\lam d {e_3}))~(\lam x x) \\
        %\t{if}~e_1~\t{then}~e_2 &\defeq&
              %\ife{e_1}{e_2}{0} \\
        %\letin{x}{e_1}{e_2}   &\defeq& (\lam x e_2)~e_1 \\
        %%e_1~;~e_2 &\defeq& \letin{x}{e_1}{e_2}, x\not\in\fun{FV}(e_2)\\
        %e_1 ~\policyAdd~ e_2 & \defeq & \lam x {e_1~x~\wedge~e_2~x} \\
        %e_1 ~\wedge~ e_2 & \defeq & \ife{e_1}{e_2}{\false} \\
%\end{array}
%\]
\end{figure}



==> standard_facet_rules_old.tex <==
\[
\begin{array}{rclcl}
\multicolumn{5}{l}{\textbf{Runtime Syntax}}\\
  e       &\in & \fun{Expr}  &::=& ... \ors a \ors \jtable{T}\\
  \Sigma  &\in & \fun{Store} &=&  (\fun{Addr} \rightarrow_p \fun{Val})
                  ~\cup~ (\fun{Label} \rightarrow \fun{Val}) \\
  R       &\in & \URawValue  &::=& c ~|~ a ~|~ \lamc{x}{\ue} \\
  a       &\in & \fun{Address} \\
  % Faceted values.
  F       &\in & \fun{Faceted Value} &::=& R \ors \labval{k}{F_1}{F_2}\\
  % Tables.
  T       &\in & \fun{Table} & = & (\USignedLabels \times \UString^n)^*\\
  % Values.
  \uv     &\in & \UValue &::=& F \ors \jtable{T}\\ 
  b       &\in & \USignedLabel &::=& k ~|~ \notlab k \\
  \pc, B  &\in & \USignedLabels &::=& b^*\\
\end{array}\\
%%
\begin{array}{lcl}
\multicolumn{3}{l}{\textbf{Evaluation Contexts}}\\
E &::=& \labval{k}{E}{e} \ors \labval{k}{V}{E}\\
  &\ors& \ctxthole \ e \ors v \ \ctxthole \ors \mkref \ctxthole \ors \deref \ctxthole \ors \assign \ctxthole e \\
  &\ors& \assign V \ctxthole \ors \row {V \dots \ctxthole e \dots} \ors \select{i}{j}{\ctxthole} \ors \project{\overline{i}}{\ctxthole}\\
  &\ors& \join{\ctxthole}{e} \ors \join{V}{\ctxthole} \ors \union{\ctxthole}{e} \ors \union{V}{\ctxthole}\\
  &\ors& \fold{\ctxthole}{e}{e} \ors \fold{V}{\ctxthole}{e} \ors \fold{V}{V}{\ctxthole}\\
\multicolumn{3}{l}{\textbf{Strict Contexts}}\\
S &::=& \ctxthole \ e \ors \deref \ctxthole \ors \assign{\ctxthole}{V} \ors \select{i}{j}{\ctxthole} \ors \project{i}{\ctxthole}\\
  &\ors& \join{\ctxthole}{V} \ors \join{\jtable T}{\ctxthole} \ors \union{\ctxthole}{V}\\ 
  &\ors& \union{\jtable{T}}{\ctxthole} \ors \row {V \dots \ctxthole e \dots}\\
  &\ors& \fold{V}{V}{\ctxthole}\\
\end{array}
\]
%%
{\bf Expression Evaluation Rules for \corelang Subset~~~ \fbox{$\sstep \Sigma e {\pc} {\Sigma'} V$}}
\[
\begin{array}{rclcl}
\setuprulecol
% F-VAL % 
\mmrule{f-val}{
  }{
    \sstep \Sigma \uv {\pc} \Sigma {\uv} 
  }
% F-REF
\mmrule{f-ref}{
    a \not\in \fun{dom}(\Sigma) \qquad
    \Sigma' = \Sigma[a := \labResult{pc}{V}{0}]\\
  }{
    \sstep \Sigma {\mkref{V}} {pc} {\Sigma'} a
  }
% F-DEREF
\mmrule{f-deref-null}{
    a \not\in \fun{dom}(\Sigma)\\
  }{
    \sstep \Sigma {\deref{a}} {pc} {\Sigma} {0}
  }
\mmrule{f-deref}{

  }{
    \sstep \Sigma {\deref{a}} {pc} \Sigma {\Sigma(a)}
  }
% F-ASSIGN
\mmrule{f-assign}{
    \Sigma' = \Sigma[a := \labResult{pc}{V}{\Sigma(a)}]
  }{
    \sstep \Sigma {a := V} {pc} {\Sigma'} V
  }
%%
\mmrule{f-ctxt}{
    E \neq [] \qquad e \mbox{ not a value}\\
    \sstep \Sigma e {pc} {\Sigma'} {V'} \qquad
    \sstep {\Sigma'} {\ctxteval{E}{V'}} {pc} {\Sigma''} {V''}\\
  }{
    \sstep \Sigma {\ctxteval{E}{e}} {pc} {\Sigma''} {V''}
  }
\end{array}
\quad\quad
%%
\begin{array}{rclcl}
\setuprulecol
% F-APP
\mmrule{f-app}{
  \sstep \Sigma {e[x := V]} {pc} {\Sigma'} {V'}
}{
  \sstep \Sigma {(\lambda x.e) \ V} {pc} {\Sigma'} {V'}
}
\mmrule{f-split}{
    k \not\in\pc~ \qquad \notlab k \not\in\pc \\
    \sstep {\Sigma} {e_1} {\joinLab k \pc} {\Sigma_1} {V_1} \\
    \sstep {\Sigma_1} {e_2} {\joinLab {\notlab k} \pc} {\Sigma'}{V_2} \\
    V' = {\labResult{k}{V_1}{V_2}} \\
  }{
    %\sstep \Sigma {\labexpr{k}{e_1}{e_2}} \pc {\Sigma'} {\labResult{k}{V_1}{V_2}}
    \sstep \Sigma {\labexpr{k}{e_1}{e_2}} \pc {\Sigma'} {V'}
  }
\mmrule{f-left}{
    k \in\pc \qquad
    \sstep \Sigma {e_1} \pc {\Sigma'} {V} \\
  }{
    \sstep \Sigma {\labexpr{k}{e_1}{e_2}} \pc {\Sigma'} V
  }
\mmrule{f-right}{
    \notlab k \in\pc \qquad
    \sstep \Sigma {e_2} \pc {\Sigma'} {V} \\
  }{
    \sstep \Sigma {\labexpr{k}{e_1}{e_2}} \pc {\Sigma'} V
  }
% F-STRICT
\mmrule{f-strict}{
    \sstep \Sigma {\labval{k}{\ctxteval{S}{V_H}}{\ctxteval{S}{V_L}}} {pc} {\Sigma'} {V'}\\
  }{
    \sstep \Sigma {\ctxteval{S}{\labval{k}{V_H}{V_L}}} {pc} {\Sigma'} {V'}
  }
\end{array}
\]


==> statement_semantics.tex <==
\begin{figure*}\caption{Faceted evaluation semantics for application and statements.{}\label{fig:appRules}\label{fig:stmtRules}\label{fig:facetencode}}
\footnotesize
{\bf Application Rules~~~ \fbox{$\appstep \Sigma {V_1~V_2 } {\pc} {\Sigma'} V'$}}
\[
\begin{array}[t]{cl}
\setuprulecol
\mrule{fa-fun}{
        	\sstep \Sigma {e[x:=V]} \pc {\Sigma'} V'
     }{
               \appstep {\Sigma} {{\lamc x e}~V} \pc {\Sigma'} {V'}
       } 
\end{array}
\qquad
\begin{array}[t]{cl}
\setuprulecol
\mrule{fa-split}{
   k \not\in \pc~ \qquad
   \notlab k \not\in \pc \\
   \appstep {\Sigma} {\Vhigh ~V_2} {\joinLab k \pc} {\Sigma_1} {\Vhigh '} \\
   \appstep {\Sigma_1} {\Vlow ~V_2} {\joinLab {\notlab k} \pc} {\Sigma'} {\Vlow'} \\
   V' = {\labResult k {\Vhigh '}{\Vlow '}}
 }{
   %\appstep {\Sigma} {\labval k {\Vhigh }{\Vlow }~V_2} \pc {\Sigma'} {\labResult k {\Vhigh '}{\Vlow '}}
   \appstep {\Sigma} {\labval k {\Vhigh }{\Vlow }~V_2} \pc {\Sigma'} {V'}
 }
\end{array}
\qquad
\begin{array}[t]{cl}
\setuprulecol
\mrule{fa-left}{
             k \in \pc \\
              \appstep {\Sigma} {\Vhigh ~V_2} \pc {\Sigma'} {V}
  }{
               \appstep {\Sigma} {\labval k {\Vhigh }{\Vlow }~V_2} \pc {\Sigma'} V
       }
\end{array}
\qquad
\begin{array}[t]{cl}
\setuprulecol
\mrule{fa-right}{
             \notlab k \in \pc \\
             \appstep {\Sigma} {\Vlow ~V_2} \pc {\Sigma'} {V}
  }{
             \appstep {\Sigma} {\labval k {\Vhigh }{\Vlow }~V_2} \pc {\Sigma'} V
       }
\end{array}
\]
%\end{figure*}
%
%
%\begin{figure*}\caption{Statement Evaluation}\label{fig:stmtRules}
{\bf Statement Evaluation Rules~~~ \fbox{$\stmtstep {\Sigma} {S} {V_p} {\fileOut{f}{R}}$}}\\
\[
\begin{array}[t]{cl}
\mrule{f-let}{
 \\
 \sstep{\Sigma}{e}{\emptyset}{\Sigma'}{V} \\
\stmtstep {\Sigma} {S[x:=V]} {V_p} {\fileOut{f}{R}} 
}{
  \stmtstep {\Sigma} {\letin{x}{e}{S}} {V_p} {\fileOut{f}{R}} 
}
\end{array}
\qquad
\begin{array}[t]{cl}
%\mrule{f-print}{
%  \sstep{\Sigma}{e_1}{\emptyset}{\Sigma_1}{V_f} \\
%  \sstep{\Sigma_1}{e_2}{\emptyset}{\Sigma_2}{V_c} \\
%  e_p = \lam x \true ~\policyAdd~ \Sigma_2(k_1) ~\policyAdd~ ... ~\policyAdd~ \Sigma_2(k_n) \\
%  \sstep{\Sigma_2}{e_p~V_f}{\emptyset}{\Sigma_3}{V_p} \\
%  \{~ k_1 ~...~ k_n ~\} ~\mbox{includes all labels in}~V_f,~V_c,~V_p \\
%  \mbox{pick}~\pc~\mbox{such that}~\pc(V_f)=f, %~~~~~~~~~~~~~~~~~~~~ \\
%    %~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%    \pc(V_c)=R,~ \pc(V_p)=\true
%}{
%  \stmtstep {\Sigma} {\print{e_1}{e_2}} {V_p} {\fileOut{f}{R}} 
%}
%\end{array}
\mrule{f-print}{
  \sstep{\Sigma}{e_1}{\emptyset}{\Sigma_1}{V_f} \\
  \sstep{\Sigma_1}{e_2}{\emptyset}{\Sigma_2}{V_c} \\
  \{~ k_1 ~...~ k_n ~\} = \fun{closeK}(\fun{labels}(e_1) ~\cup~ \fun{labels}(e_2), \Sigma_2) \\
  e_p = \lam x \true ~\policyAdd~ \Sigma_2(k_1) ~\policyAdd~ ... ~\policyAdd~ \Sigma_2(k_n) \\
  \sstep{\Sigma_2}{e_p~V_f}{\emptyset}{\Sigma_3}{V_p} \\
  \mbox{pick}~\pc~\mbox{such that}~\pc(V_f)=f,
    \pc(V_c)=R,~ \pc(V_p)=\true
}{
  \stmtstep {\Sigma} {\print{e_1}{e_2}} {V_p} {\fileOut{f}{R}}
}
\end{array}
\qquad
  \begin{array}[t]{rcl}
    \fun{closeK}(K, \Sigma) & = &
           \mbox{let}~ K' = \cupk~ \fun{labels}(\Sigma(k)) ~\mbox{in}~ \\
        && \mbox{if}~ K' = K \\
        && ~~~~\mbox{then}~ K \\
        && ~~~~\mbox{else}~ \fun{closeK}(K', \Sigma) \\
  \end{array}
\]
%{\bf Semantics for Derived Encodings}\\
%\[
%\begin{array}{cl}
%\ifrule{f-if-true}{
        %\sstep \Sigma {e_1} {\pc} {\Sigma_1} {\true}  \\
        %\sstep {\Sigma_1} {e_2} {\pc} {\Sigma'} {V}  \\
       %}{
        %\sstep \Sigma {\ife{e_1}{e_2}{e_3}} {\pc} {\Sigma'} {V} 
       %}
%\ifrule{f-if-false}{
        %\sstep \Sigma {e_1} {\pc} {\Sigma_1} {\false}  \\
        %\sstep {\Sigma_1} {e_3} {\pc} {\Sigma'} {V}  \\
       %}{
        %\sstep \Sigma {\ife{e_1}{e_2}{e_3}} {\pc} {\Sigma'} {V} 
       %}
%\end{array}
%\qquad\qquad
%\begin{array}{cl}
%\ifrule{f-if-split}{
        %\sstep \Sigma {e_1} {\pc} {\Sigma_1} {\labval{k}{V_H}{V_L}}  \\
        %e_H = {\ife{V_H}{e_2}{e_3}} \\
        %e_L = {\ife{V_L}{e_2}{e_3}} \\
        %\sstep {\Sigma_1} {\labval{k}{e_H}{e_L}} {\pc} {\Sigma'} {V}  \\
       %}{
        %\sstep \Sigma {\ife{e_1}{e_2}{e_3}} {\pc} {\Sigma'} {V} 
       %}
%\end{array}
%\]

%{\bf Auxiliary Functions}
%\[
  %\begin{array}{rcl}
    %\fun{closeK}(K, \Sigma) & = &
           %\mbox{let}~ K' = \cupk~ \fun{labels}(\Sigma(k)) ~\mbox{in}~ \\
        %&& \mbox{if}~ K' = K \\
        %&& ~~~~\mbox{then}~ K \\
        %&& ~~~~\mbox{else}~ \fun{closeK}(K', \Sigma) \\
  %\end{array}
%\]
\end{figure*}

